Chrisimos: A useful Proof-of-Work for finding Minimal Dominating Set of a graph

Hash-based Proof-of-Work (PoW) used in the Bitcoin Blockchain leads to high energy consumption and resource wastage. In this paper, we aim to re-purpose the energy by replacing the hash function with real-life problems having commercial utility. We propose Chrisimos, a useful Proof-of-Work where miners are required to find a minimal dominating set for real-life graph instances. A miner who is able to output the smallest dominating set for the given graph within the block interval time wins the mining game. We also propose a new chain selection rule that ensures the security of the scheme. Thus our protocol also realizes a decentralized minimal dominating set solver for any graph instance. We provide formal proof of correctness and show via experimental results that the block interval time is within feasible bounds of hash-based PoW.

==> related.tex <==
\section{Related Works}
\label{related}
The proof of useful work was first introduced in \cite{ball2017proofs} correlates consensus protocol hardness to solving NP-complete problems of practical interest. A mathematical formalization of the PoUW and its properties has been specified as well. Further constructions for PoUW mining were given by Loe et al. \cite{loe2018conquering}, and Dotan et al. \cite{dotan2020proofs}. In all these previous approaches the security of the system was not rigorously analyzed and in many cases, the attacker can manipulate the system by providing easy instances to solve.

A hybrid scheme for PoUW based on the traveling salesman problem (TSP) has been proposed in \cite{loe2018conquering,syafruddin2019blockchain} but the utility of the approach has not been discussed. PoUW based on machine-learning problems was suggested by \cite{baldominos2019coin} but these systems could be easily attacked. Another hybrid approach \cite{philippopoulos2020difficulty} to mining combines hash value calculations with difficulty-based incentives for problem-solving. The miners get an incentive for solving real-life problems for scientific purposes. However, the protocol is susceptible to an attack where miners find multiple solutions to a real-life instance, and instead of using the best one, they mine several blocks in a row using all the solutions. Another PoUW protocol named proof-of-search \cite{shibata2019proof} is used as a tool to find approximate solutions to any optimization problem. However, the complexity of the overall proof-of-search protocol is too large, and the system is too restrictive in terms of providing a solution. Another PoUW protocol based the doubly parallel local search (DPLS) algorithm named Ofelimos has been proposed in \cite{fitzi2022ofelimos}. DPLS represents a general-purpose stochastic local-search algorithm having a component called the exploration algorithm. The latter is used to produce a set of points in a solution space based on the given input parameters preventing miners from picking easy exploration steps and reducing the complexity of mining. However, they do not take into account the difficulty of NP-hard problem instances which might lead to unfairness while block generation. A recent work called Combinatiorial Optimization Consensus Protocol (COCP) \cite{todorovic2022proof} proposes efficient utilization of computing resources by providing valid solutions for the real-life instances of any combinatorial optimization problem. An unsolved problem present in the instance pool is selected and miners start solving for the given instance. A miner upon finding the solution sends it to a solution pool. The role of the solution pool is to keep all valid solutions for each considered instance and to enable the identification and rewarding of the miner who found the best solution. This is a major drawback because the authors assume that a centralized entity will check the solution pool and return the best solution among all. This assumption may lead to problems if the entity running the solution retrieval module on this pool is malicious and tends to favor a solution from a particular miner.

Our protocol overcomes the drawbacks observed in the state-of-the-art useful Proof-of-Work. Unlike in \cite{fitzi2022ofelimos}, we do not consider pool mining in our solution. Introducing pool of miners will make our system fair as miners will be rewarded for their contribution. As a part of future work, we would explore pool mining for \emph{Chrisimos}.  

